Automatic transformation of irreducible representations for efficient contraction of tensors with cyclic group symmetry

Tensor contractions are ubiquitous in computational chemistry and physics, where tensors generally represent states or operators and contractions express the algebra of these quantities. In this context, the states and operators often preserve physical conservation laws, which are manifested as group symmetries in the tensors. These group symmetries imply that each tensor has block sparsity and can be stored in a reduced form. For nontrivial contractions, the memory footprint and cost are lowered, respectively, by a linear and a quadratic factor in the number of symmetry sectors. State-of-the-art tensor contraction software libraries exploit this opportunity by iterating over blocks or using general block-sparse tensor representations. Both approaches entail overhead in performance and code complexity. With intuition aided by tensor diagrams, we present a technique, irreducible representation alignment, which enables efficient handling of Abelian group symmetries via only dense tensors, by using contraction-specific reduced forms. This technique yields a general algorithm for arbitrary group symmetric contractions, which we implement in Python and apply to a variety of representative contractions from quantum chemistry and tensor network methods. As a consequence of relying on only dense tensor contractions, we can easily make use of efficient batched matrix multiplication via Intel's MKL and distributed tensor contraction via the Cyclops library, achieving good efficiency and parallel scalability on up to 4096 Knights Landing cores of a supercomputer.

==> algebraic.tex <==
\subsection{Formal Derivation}

\begin{figure*}[h]
\centering
\includegraphics[width=\textwidth]{diagrams/detailed_contraction_annotated}
\caption{Derivation of transformations necessary for efficient contraction algorithm of order 4 tensors with group symmetry. Thick lines may correspond to any number of indices, including 0.}
\label{fig:irrep_ord4_contraction}
\end{figure*}

{\color{red}It would be nice if someone could ensure that the diagrams in the previous section encode all the above diagrams. Also (although presumably more   work) it would be nice if the equations in this and the previous section are in correspondence with each other. Otherwise notation should be consistent.}
We now provide an algorithm to do this transformation for an arbitrary tensor contraction with group symmetric tensors, demonstrate correctness, and quantify costs.
All steps of the algorithms and the Lemmas used to define the transformations ad described by tensor diagrams in Figure~\ref{fig:irrep_ord4_contraction}.

Consider tensors $\tsr{T}\in\{\tsr{U},\tsr{V},\tsr{W}\}$, where $\tsr{T}\in\mathbb{C}^{K_1\times\cdots\times K_N}$ has a cyclic group symmetry, 
Any contraction of tensors $\tsr{U}$ and $\tsr{V}$ into $\tsr{W}$ can be written as
\begin{align}
w_{a\vcr{b}i\vcr{j}} = \sum_{k,\vcr{l}} u_{a\vcr{b}k\vcr{l}} v_{k\vcr{l}i\vcr{j}}, \label{eq:naive_ctr}
\end{align}
where $\vcr{b}$, $\vcr{j}$, and $\vcr{l}$ are collections of multiple indices.
%Assume for simplicity that each index ranges from $1$ to $n$.
For simplicity of presentation, we assume these index collections are all of size $M$ and that each tensor is equidimensional (so all modes/indices have same size, $K_1=\cdots = K_{N}= n$ with $N=2(M+1)$).
Our results extend naturally to the cases when the three collections contain different numbers of indices and the tensor modes have different dimensions.
If each $\tsr{T}\in\{\tsr{U},\tsr{V},\tsr{W}\}$, where $\tsr{T}\in\mathbb{C}^{n\times\cdots\times n}$ has a cyclic group symmetry, 
we can express it in terms of a \emph{irreducible representation} $\tsr{\hat{T}}$ and a \emph{group tensor} $\dlt T$ that is described by an coefficient vector $\coeff T \in \mathbb{Z}^{N}$, so
%with $N=2(M+1)$, so that,
%and remainder $\rem T\in\{0,\ldots, n-1\}$
\begin{align}
t_{i\vcr{j}} = \hat{t}_{\vcr{j}}\edlt{T}_{i\vcr{j}},\ \text{where}\
  \edlt{T}_{i\vcr{j}}&=\begin{cases} 1 & : \langle \coeff{T}, i\vcr j \rangle  \equiv  \rem T \mod n \\ 0 & : \text{otherwise} \end{cases}, \label{eq:delta} \\
\text{in which} \ \langle\coeff{T}, i\vcr j \rangle &= \ecoeff{T}_1 i + \ecoeff{T}_2 j_1 + \cdots + \ecoeff{T}_{N}j_{N-1}.
\end{align}
We denote the set of possible $\tsr{\delta}$ tensors (choices of coefficient vectors $\mathbb{Z}^{N}$ and dimension $n$) as $\mathbb{D}_{(n,N)}$.
We may similarly isolate any other index in $\tsr{T}$ in place of the first index $i$.
Using \eqref{eq:delta}, we can expand \eqref{eq:naive_ctr} as
\begin{align}
w_{a\vcr{b}i\vcr{j}} = \sum_{k,\vcr{l}} \hat{u}_{\vcr{b}k\vcr{l}}\edlt{U}_{a\vcr{b}k\vcr{l}}\edlt{V}_{k\vcr{l}i\vcr{j}} \hat{v}_{k\vcr{l}\vcr{j}}. \label{eq:irrep_naive_ctr}
\end{align}
To devise an algorithm for efficient contraction of group-symmetric tensors, we first introduce a few transformation rules for the group tensors.
\begin{lemma}
\label{lem:t1}
Given two group tensors $\dlt{X}, \dlt{Y} \in \mathbb D_{(n,N)}$ with coefficient vectors $\coeff X = \begin{bmatrix} \coeff 1 \\ \coeff 2 \end{bmatrix}$ and $\coeff Y = \begin{bmatrix} \coeff 2 \\ \coeff 3 \end{bmatrix}$, we have
\begin{align}
\edlt{X}_{a\vcr{b}k\vcr{l}}\edlt{Y}_{k\vcr{l}i\vcr{j}} = \sum_{q=1}^{n} \edlt{A}_{a\vcr{b}q}\edlt{B}_{k\vcr{l}q}\edlt{C}_{i\vcr{j}q},\label{eq:lemma1}
\end{align}
where $\dlt{A},\dlt{B},\dlt{C}\in \mathbb D_{(n,N-M)}$ have coefficient vectors 
$\coeff A = \begin{bmatrix} \coeff{1} \\ 1 \end{bmatrix}$,
$\coeff B = \begin{bmatrix} \coeff{2} \\ -1 \end{bmatrix}$, and
$\coeff C = \begin{bmatrix} \coeff{3} \\ 1 \end{bmatrix}$.
\end{lemma}
\begin{proof}
%=$\rem{A}=-\rem{Y}$, $\rem{B}=\rem{X}+\rem{Y}$, $\rem{C} = -\rem{X}$ so that 
$\edlt{A}_{a\vcr{b}q}\edlt{B}_{k\vcr{l}q}\edlt{C}_{i\vcr{j}q}=1$ whenever all of the following hold,
\begin{align*}
\langle \coeff{1},a\vcr{b}\rangle  & \equiv q \mod n, \\
\langle \coeff{2},k\vcr{l}\rangle 
 & \equiv -q \mod n, \\
\langle \coeff{3},i\vcr{j}\rangle   & \equiv q \mod n.
\end{align*}
These conditions are true for at most a single $q\in\{1,\ldots,n\}$ given a choice of $a\vcr{b}i\vcr{j}k\vcr{l}$.
Further, we have that $\sum_{q=1}^{n} \edlt{A}_{a\vcr{b}q}\edlt{B}_{k\vcr{l}q}\edlt{C}_{i\vcr{j}q}=1$,
whenever the following two conditions hold,
\begin{align*}
\underbrace{\langle \coeff{1},a\vcr{b}\rangle + \langle \coeff{2},k\vcr{l}\rangle }_{
 \langle \coeff{X},a\vcr b k \vcr l \rangle} & \equiv 0 \mod n, \\
\underbrace{ \langle \coeff{2},k\vcr{l}\rangle + \langle \coeff{3},i\vcr{j}\rangle }_{
 \langle \coeff{Y},k \vcr l i \vcr j\rangle}  & \equiv 0 \mod n.
\end{align*}
These conditions hold if and only if $\edlt{X}_{a\vcr{b}k\vcr{l}}\edlt{Y}_{k\vcr{l}i\vcr{j}}=1$ as the latter implies $\edlt{X}_{a\vcr{b}k\vcr{l}}=\edlt{Y}_{k\vcr{l}i\vcr{j}}=1$.
\end{proof}
\begin{lemma}
\label{lem:t2}
Consider any tensor $\tsr{\hat{X}}$ and any group tensor $\dlt{X} \in \mathbb D_{(n,N)}$. Let $\hat{y}_{j\vcr{k}} = \sum_l \edlt{X}_{lj\vcr{k}}\hat{x}_{l \vcr k}$, then %and $\dlt{Y} \in \mathbb D_{(n,N)}$, such that
\[\edlt{X}_{ij\vcr{k}}\hat{x}_{i \vcr k} = \edlt{X}_{ij\vcr{k}}\hat{y}_{j\vcr{k} }.\]
\end{lemma}
\begin{proof}
When $\edlt{X}_{ij\vcr{k}}=1$, we have that for $l\neq i$, $\edlt{X}_{lj\vcr{k}}=0$ {\color{red} does this still work when $\ecoeff{X}_i>1$? Perhaps dimensions need to be adjusted accordingly in that case} so
\[\edlt{X}_{ij\vcr{k}}\hat{y}_{j\vcr{k}} = \edlt{X}_{ij\vcr{k}}\sum_l \edlt{X}_{lj\vcr{k}}\hat{x}_{l \vcr k}=\edlt{X}_{ij\vcr{k}}\edlt{X}_{ij\vcr{k}}\hat{x}_{i \vcr k}=\edlt{X}_{ij\vcr{k}}\hat{x}_{i \vcr k}.\]
%
%Let $\pi_{ijst}=1$ when $(i,j)=(s,t)$, so that $\pi_{ijst}w_{ij} =\pi_{ijst}w_{ts}$ and note that 
%\[\sum_{st}\pi_{ijst}\pi_{stmn} = \delta_{ij,mn} = \begin{cases} 1 & : i=m,j=n \\ 0 & : \text{otherwise}\end{cases},\]
%then we have that
%\[\edlt{X}_{ij\vcr{k}}\hat{x}_{i \vcr k} = \sum_{stmn} \edlt{X}_{ij\vcr{k}}\pi_{ijst}\pi_{stmn}\hat{x}_{m \vcr k}\]
%
%\[x_{ij\vcr{k}} = \edlt{X}_{ij\vcr{k}}\hat{x}_{i \vcr k} = \begin{cases} \hat x_{i\vcr{k}} & : \ecoeff{X}_1 i + \ecoeff{X}_2 j + \langle \coeff{X}_3, \vcr{k} \rangle \equiv 0 \mod n\\
%0 & : \text{otherwise}
%\end{cases}.
%\]
%Using $\coeff{Y}{} = \begin{bmatrix} -\ecoeff{X}_2 & -\ecoeff{X}_1 & \coeff{X}_3{} \end{bmatrix}$, we can note that
%\[\edlt{Y}_{ij\vcr{k}}\hat{x}_{j\vcr{k} } = \begin{cases} \hat y_{j\vcr{k}} & : 
%  %\ecoeff{Y}_1 i + \ecoeff{Y}_2 j + \langle \coeff{Y}_3, \vcr{k} \rangle 
%  = -\ecoeff{X}_2 i -\ecoeff{X}_1 j + \langle \coeff{X}_3, \vcr{k} \rangle \equiv 0 \mod n\\
%0 & : \text{otherwise}
%\end{cases}
%\]
%also yields $x_{ij\vcr{k}}$.
\end{proof}

Our algorithm rewrites the tensor contraction in~\eqref{eq:naive_ctr} as
\begin{align*}
w_{a\vcr{b}i\vcr{j}} = \sum_{k,\vcr{l}} \hat{u}_{\vcr{b}k\vcr{l}}\sum_{q=1}^{n} \edlt{A}_{a\vcr{b}q}\edlt{B}_{k\vcr{l}q}\edlt{C}_{i\vcr{j}q} \hat{v}_{k\vcr{l}\vcr{j}},
\end{align*}
which is possible due to Lemma~\ref{lem:t1}.
Now, we further transform the contraction expression by substituting in $\hat{y}_{\vcr{b}q\vcr{l}}=\sum_s \edlt{B}_{s\vcr{l}q}\hat{u}_{\vcr{b}s\vcr{l}}$ to obtain
\begin{align*}
w_{a\vcr{b}i\vcr{j}} = \sum_{k,\vcr{l}}\sum_{q=1}^{n} \hat{y}_{\vcr{b}q\vcr{l}} \edlt{A}_{a\vcr{b}q}\edlt{B}_{k\vcr{l}q}\edlt{C}_{i\vcr{j}q} \hat{v}_{k\vcr{l}\vcr{j}},
\end{align*}
which holds due to the following Lemma~\ref{lem:t2}.
We can then compute $z_{q\vcr{l}\vcr{j}}=\sum_k\edlt{B}_{k\vcr{l}q}\hat{v}_{k\vcr{l}\vcr{j}}$ and obtain
\begin{align*}
w_{a\vcr{b}i\vcr{j}} &= \sum_{\vcr{l}}\sum_{q=1}^{n} \hat{y}_{\vcr{b}q\vcr{l}} \edlt{A}_{a\vcr{b}q}\edlt{C}_{i\vcr{j}q} \hat{z}_{q\vcr{l}\vcr{j}} \\
&= \sum_{q=1}^{n}\edlt{A}_{a\vcr{b}q}\edlt{C}_{i\vcr{j}q}\underbrace{\sum_{\vcr{l}} \hat{y}_{\vcr{b}q\vcr{l}}  \hat{z}_{q\vcr{l}\vcr{j}}}_{\hat{x}_{q\vcr b\vcr j}} 
\end{align*}
Then using Lemma~\ref{lem:t2} again to get $\edlt{C}_{i\vcr{j}q}\hat{w}_{i\vcr b\vcr j} = \edlt{C}_{i\vcr{j}q}\hat{x}_{q\vcr b\vcr j}$, where $\hat{w}_{i\vcr b\vcr j}=\sum_r\edlt{C}_{i\vcr{j}r}\hat{x}_{r\vcr b \vcr j}$ is the irreducible representation of $\tsr{W}$, since
\begin{align*}
w_{a\vcr{b}i\vcr{j}} &= 
 \underbrace{\sum_{q=1}^{n}\edlt{A}_{a\vcr{b}q}\edlt{C}_{i\vcr{j}q}}_{\edlt{W}_{a\vcr b i\vcr j}}\hat{w}_{i\vcr b\vcr j}.
\end{align*}
The above derivation demonstrates correctness.
We summarize the computational steps below.
\begin{enumerate}
\item Take as input $\tsr{\hat{U}}$, $\tsr{\hat{V}}$ and coefficient vectors $\coeff{U}=\begin{bmatrix} \coeff{1} \\ \coeff{2} \end{bmatrix}$, $\coeff{V}=\begin{bmatrix} \coeff{2} \\ \coeff{3} \end{bmatrix}$ that define group tensors $\dlt{U}$, $\dlt{V}$.
\item Compute $\tsr{Y}$ so that $\hat{y}_{\vcr{b}q\vcr{l}}=\sum_s \edlt{B}_{s\vcr{l}q}\hat{u}_{\vcr{b}s\vcr{l}}$ where $\dlt{B}$ has coefficient vector $\begin{bmatrix} \coeff{2} \\ -1 \end{bmatrix}$
\item Compute $\tsr{Z}$ so that $z_{q\vcr{l}\vcr{j}}=\sum_k\edlt{B}_{k\vcr{l}q}\hat{v}_{k\vcr{l}\vcr{j}}$.
% where $\dlt{B}$ has coefficient vector $\begin{bmatrix} \coeff{2} \\ -1 \end{bmatrix}$.
\item Compute $\tsr{\hat{X}}$ so that $\hat{x}_{q\vcr b\vcr j} = \sum_{\vcr{l}} \hat{y}_{\vcr{b}q\vcr{l}}  \hat{z}_{q\vcr{l}\vcr{j}}$.
\item Compute $\tsr{\hat{W}}$ so that $\hat{w}_{i\vcr b\vcr j}=\sum_r\edlt{C}_{i\vcr{j}r}\hat{x}_{r\vcr b \vcr j}$ where $\dlt{C}$ has coefficient vector $\begin{bmatrix}\coeff 3 \\ 1 \end{bmatrix}$.
\item Output $\tsr{\hat{W}}$ so that together with coefficient vector {\color{red} check formally that this coefficient vector is correct} $\coeff{W}=\begin{bmatrix} \coeff 1 \\ \coeff{3} \end{bmatrix}$ defining $\dlt{W}$, we have
\[\underbrace{\edlt{W}_{a\vcr b i\vcr j}\hat{w}_{i\vcr b\vcr j}}_{w_{a\vcr{b}i\vcr{j}}}
= \sum_{k\vcr l}
  \underbrace{\edlt{U}_{a\vcr b k\vcr l}\hat{u}_{\vcr b k \vcr l}}_{u_{a\vcr{b}k\vcr{l}}}
  \underbrace{\edlt{V}_{k\vcr l i\vcr j}\hat{v}_{k\vcr l\vcr j}}_{v_{k\vcr{l}i\vcr{j}}}.\]
\end{enumerate}
Steps 2, 3, and 5, can be done with cost $O(n^{2M+1)})$, i.e., linear in the size of the irreducible representation of the inputs $\tsr{U}$, $\tsr{V}$, and the output $\tsr{W}$, respectively, by leveraging the sparsity of the group tensors.
These operations can alternatively be performed as dense tensor contractions with a factor of $n$ more cost.
The cost of step 4 and of the algorithm overall is $O(n^{3M+1})$, a factor of $\Theta(n^2)$ less than naive contraction.


==> graphical_alg.tex <==
We now describe  the general algorithm and irrep alignment transformation using intuitive
diagrammatic arguments. To do so, we introduce a graphical notation to represent cyclic group tensors, their
irreps {\color{red}two kinds of irreps used now: standard irrep form, irrep aligned form}, and their tensor contractions.
This notation is derived from that used in Feynman diagrams and in the theory of tensor networks. {\color{red}Also change all equations
  if we are using vector indices.}

\begin{figure*}[h]
\centering
\includegraphics[width=.5\textwidth]{diagrams/Figx1}
\caption{Left: tensor with modes unfolded into physical modes (lowercase letters) and symmetry modes (arrows, labelled by uppercase letters). The
  direction of the arrows indicates the conservation rule, here $A+B+C=D+E+F$. Right: standard irrep form of tensor, where one of the symmetry modes
  is fixed by the conservation rule, thus one arrow is deleted.}
\label{fig:x1}
\end{figure*}


A tensor of order $r$ will be denoted by an object with $r$ legs, as shown in Fig.~\ref{fig:x1}. Labelling all
of the legs indexes a single element of the tensor. As in Eq.~\ref{eq:unfolded},
we can unfold the modes of a cyclic group tensor to obtain symmetry modes (irreps) and physical modes,
and in graphical form, we introduce arrows to label the symmetry modes. The direction of the arrow
serves to define the sign associated with the conservation law, e.g. in Fig.~\ref{fig:x1} for the tensor $\mathcal{T}$ with
elements $t_{aA,bB,cD,dD,eE,fF}$ the sum of all ingoing arrows equals the sum of all outgoing arrows, thus
\begin{align}
  A + B + C - D - E - F \mod G = 0
  \end{align}
Because each tensor is symmetric, one of its symmetry labels is redundant. Consequently, we can delete any
of the symmetry labels in Fig.~\ref{fig:x1} and still uniquely index the tensor. This is
shown in Fig.~\ref{fig:x1} where one of the arrows has been deleted. We refer to this non-redundant labelling of
the tensor elements as the standard irrep form.

To efficiently contract two cyclic group tensors $\mathcal{S}, \mathcal{T}$, we convert each tensor
into the irrep aligned form, another reduced representation. To understand the structure of this form,
we formally carry out a singular value decomposition (SVD) on each tensor between the modes that
will be contracted (contracting modes) and the uncontracted modes. Graphically, we represent this
by pulling apart each tensor into two tensors as shown in Fig.~\ref{fig:x2}, joined by a new symmetry mode $Q$.
For example, if the contracted modes are $cC, fF$, Fig.~\ref{fig:x2} represents for tensor $\mathcal{T}$
\begin{align}
  t_{aA,bB,cC,dD,eE,fF} = \sum_{Q} u_{aA,bB,cC,Q} \sigma_Q v_{Q,dD,eE,fF} =\sum_{Q} \tilde{u}_{aA,bB,cC,Q}  \tilde{v}_{Q,dD,eE,fF} \notag\\
  \end{align}
where we grouped the singular values into the definition of the tensors $\tilde{u}$, $\tilde{v}$.
Note that the new mode $Q$ has no associated physical mode.
$\tilde{u}$ and $\tilde{v}$ are themselves cyclic group tensors
thus we can remove any one of the symmetry labels from them,
\begin{align}
  \tilde{u}_{aA,bB,cC,Q}  \to   \tilde{u}_{a,bB,cC,Q}
  \tilde{v}_{Q,dD,eE,fF} \to   \tilde{v}_{Q,dD,eE,f}
  \end{align}
and multiplied together, these define the irrep aligned form of $\mathcal{T}$,
\begin{align}
    t_{aA,bB,cC,dD,eE,fF} \to \hat{t}_{a,bB,cC,dD,eE,f,Q} = \tilde{u}_{a,bB,cC,Q} \tilde{v}_{Q,dD,eE,f}
\end{align}
Graphically, the irrep aligned form of the tensor is represented by a diagram where two symmetry arrows (one from
the contracting modes, one from the uncontracted modes) have been removed.
Note that the irrep aligned form does not actually require an SVD to be performed. Instead, one can assign the elements of
$\mathcal{T}$ as (see Fig.~\ref{fig:x2} for directions of arrows)
\begin{align}
  \hat{t}_{a,bB,cC,dD,eE,f,Q} = t_{aA,bB,cC,dD,eE,fF} \  \mathrm{ if}  \ A + B + Q = D + E, Q+F=C \! \pmod G \label{eq:irrepassign}
  \end{align}
Thus to show that the splitting of the tensor into two is not actually performed, and also that $Q$ is an internal symmetry
mode not associated with a physical mode, we use the graphical notation in Fig.~\ref{fig:x3} where $Q$ as an internal leg connecting
two formal internal vertices of $\mathcal{T}$.
In practice, the assignment in Eq.~\ref{eq:irrepassign} can be implemented efficiently by  contracting with Kronecker tensors, e.g.
\begin{align}
  \hat{t}_{a,bB,cC,dD,eE,f,Q} = \sum_{AF} t_{aA,bB,cC,dD,eE,fF} \delta_{A+B+Q,D+E} \delta_{Q+F,C}
\end{align}

\begin{figure*}[h]
\centering
\includegraphics[width=.9\textwidth]{diagrams/Figx2}
\caption{Left: a tensor can be converted into the irrep aligned form by a formal splitting between the modes that are contracting
  and the modes that are left uncontracted. Center: The split form introduces a new symmetry label ($Q$) and this induces two
  conservation rules at each of the split vertices, which allows us to delete two symmetry labels. Right:  Symmetry label $Q$ is internal to the irrep aligned tensor and is not associated with a physical mode. {\color{red} Y - I think it would be nice to add labels $t, \hat{t}$, $\mu$, $\nu$ in the circles}}
\label{fig:x2}
\end{figure*}


\begin{figure*}[h]
\centering
\includegraphics[width=\textwidth]{diagrams/Figx3}
\caption{Left: Once transformed into irrep aligned form, two cyclic group symmetric tensors can be
  contracted via dense matrix multiplication and a summation over the internal symmetry mode $Q$. Right: the final
  contracted tensor can be converted into standard irrep form, eliminating $Q$ using conservation rules at the two internal
  vertices.}
\label{fig:x3}
\end{figure*}


Once both tensors $\mathcal{S}$, $\mathcal{T}$ are in irrep aligned form, the contraction between them for
each common irrep $Q$ can proceed as a dense tensor contraction. This is shown in
Fig.~\ref{fig:x3}, representing the contraction
\begin{align}
  \hat{x}_{a, f, iI,jJ,hH,gG, Q} =\sum_{c,dD,eE} \hat{s}_{a,c,dD,eE,iI,jJ,Q} \hat{t}_{c,dD,eE,f,hH,gG,Q}
  \end{align}
The internal symmetry mode $Q$ must be the same on each tensor for a non-zero contribution
due to the contraction lemma shown in Fig.~\ref{fig:x4}. Because
two of the modes of the output tensor $\mathcal{X}$ have no symmetry mode, and one of the contracted modes has no symmetry mode, while
the above operation must be performed for each $Q$, the total arithmetic cost is reduced by a factor
of $G^2$. Finally, the output tensor $\mathcal{X}$ can be converted back into other representations, such as the standard irrep
form using the conservation rules at each of the internal vertices of $\mathcal{X}$, as shown in Fig.~\ref{fig:x3}.

\begin{figure*}[h]
\centering
\includegraphics[width=.7\textwidth]{diagrams/Figx4}
\caption{Contraction lemma: the outgoing symmetry labels from any contraction must be the same for non-zero values
  due to conservation at each of the vertices.}
\label{fig:x4}
\end{figure*}


==> motiv.tex <==

Cyclic group tensors arise in a variety of settings in computational quantum chemistry and physics methods.
This is because both the quantum Hamiltonian and its eigenstates transform as irreps of
the physical symmetry operators, for example, those associated with particle number,
spin, and point group and lattice symmetries~\cite{lax2001symmetry,cotton2003chemical,sternberg1995group}. Many of these symmetries
are associated with finite
cyclic groups (e.g. finite Abelian point groups or finite lattice groups) or infinite cyclic groups (e.g. particle number
symmetry and magnetic spin symmetry). %Those associated with infinite cyclic groups give rise to conservation laws
%via Noether's theorem.

%% for modelling quantum systems, in computational chemistry and condensced matter physics applications.
In this section, we summarize some of the quantum chemistry and physics applications
of cyclic group tensors, and related developments to handle cyclic group symmetry within them.
The performance evaluation of our proposed algorithms later considers some of the computationally expensive
tensor contractions arising in these applications.

\subsection{Electronic Structure}

In electronic structure calculations in  chemistry and physics, the Hamiltonian can be written as order 4 and order 2 tensors using discretized basis. %the most complicated
%part of the discretized Hamiltonian can be written as an order 4 tensor, often called the
%\emph{two-electron integral tensor}. 
Similarly, the many-body eigenstates and wavefunctions are represented by tensors. One common choice of approximate wavefunction, arising in so-called correlated wavefunction methods such
as configuration interaction (CI)~\cite{szabo2012modern} and coupled cluster methods at the doubles level of approximation~\cite{cizek_paldus71,cizek66,crawford_intro,Gauss:2002:ECC:CC,Bartlett:2007:RMP:CC}, represents an important part of the wavefunction in terms of
another order 4 tensor, the  \emph{doubles amplitude tensor}. Higher order tensors arise in approximations that target higher accuracy~\cite{purvis_bartlett82,Stanton:1997:CPL:whyCCSD(T),Kallay:2001:JCP:generalCC,Noga:1987:JCP:CCSDT}.

%% are prevalent in wavefunction-based methods for electronic structure calculatons in quantum chemistry
%% These, `second-quantized' methods, discretize the Hamiltonian operator via an order 4
%% Some methods, such as the family of
%%  methods~\cite{szalay2012multiconfiguration} and coupled-cluster (CC) methods~\cite{cizek_paldus71,cizek66,crawford_intro,Gauss:2002:ECC:CC,Bartlett:2007:RMP:CC} also work with \emph{amplitude tensors}, which are used to represent the wavefunction (some approximation of a desired state, e.g. the ground state).
%%  Order 4 amplitude tensors are most commonly used~\cite{Scuseria:JCP:1988:CCSDfactorize,Scuseria:JCP:1989:CCvQCI}, but higher-order
%%  variants arise in more methods that seek higher accuracy~\cite{purvis_bartlett82,Stanton:1997:CPL:whyCCSD(T),Kallay:2001:JCP:generalCC,Noga:1987:JCP:CCSDT,Scuseria:1988:CPL:CCSDT} or compute additional properties, such as gradients~\cite{Krylov:2008:ARPC:EOMCC,kowalski:7411,Stanton:1993:JCP:EOMCC}.

Both the Hamiltonian tensor and the wavefunction tensors possess the cyclic group symmetries associated with
the physical symmetries of the system. In a molecule, the largest symmetry group for which
cost reductions can be achieved is usually the \emph{point group symmetry}, e.g. associated with a rotational group $C_{nv}$  or a product group such as $D_{2h}$.
In crystalline materials, crystal translational symmetry is equivalent to a cyclic symmetry along each lattice direction. Typically the cyclic groups (number of $k$-points) are chosen to be as large as computationally feasible. Thus the savings arising from efficient use of translational symmetry are particularly important in materials simulations~\cite{mcclain2017gaussian,hirata2004coupled,hummel2017low,flocke2003correlation,motta2019hamiltonian}.

%% if the systemmolecule under consideration has \emph{point-group symmetry}, e.g., rotational symmetry~\cite{vcarsky1987use}, which is common for many molecules of interest for electronic structure calculations.
%% Additional cyclic symmetry structure arises in periodic formulations of these methods, which are affective given regular/repeating sturcture common in solid state modelling.

Many quantum chemistry implementations leverage cyclic group symmetries within various
approximate quantum methods~\cite{scuseria1987closed,stanton1991direct,mcclain2017gaussian}.
%% , including configuration interaction~\cite{scuseria1987closed,}, M{\o}ller-Plessert perturbation theory~\cite{moller1934note,stanton1991direct}, and coupled cluster~\cite{scuseria1987closed,stanton1991direct,matthews2019extending}.
%% Reports of improvements of performance of up to 30x due to use of cyclic group symmetry date back to the 1980s~\cite{scuseria1987closed}.
In addition, a number of state-of-the-art tensor software efforts aimed at quantum chemistry applications handle cyclic group symmetry in a general way via block sparse tensor formats~\cite{ozog2013inspector,lai2013framework,peng2016massively,ibrahim2014analysis,Kendall2000260,doi:10.1021/jp034596z,springerlink_ga1}.
As described in Section~\ref{subsec:symalg_ex}, our proposed algorithm achieves the same computational improvement via
transforming the cyclic group tensor representation, while maintaining a global view of the problem
as a dense tensor contraction, as opposed to a series of block-wise operations or a contraction of block-sparse tensors. 

\subsection{Tensor Network Simulation}

%Tensor network methods model a quantum state and Hamiltonians that operate on the state as a contraction of many tensors (\emph{sites}), each of which is much smaller than the tensors directly describing the state and Hamiltonian.
%A \emph{matrix product state (MPS)} (also refered to as a \emph{tensor train}~\cite{}), which is a 1D tensor network, is most widely used, especially as part of the \emph{density matrix renormalization group (DMRG)} method~\cite{}.
%DMRG uses alternating optimization of a 1D tensor network to arrive at representations of ground-states or excited states of a quantum system described by a Hamiltonian that is itself represented as a tensor train (\emph{matrix product operator (MPO)}~\cite{hubig2017generic}).
%Physical Hamiltonians satisfy conservation laws, which result in cyclic group symmetries within the MPS and MPO.
%Specifically, \emph{quantum number symmetries} may be used to represent conservation of ... ~\cite{}.
%
%Tensor networks that go beyond 1D may have substantially more expressive power~\cite{verstraete2004peps,ye2018tensor}.
%In particular, 2D tensors networks, \emph{projected entangled pair states (PEPS)} and associated operators (PEPOs), provide a more compact representation of many Hamiltonians of physical interest~\cite{verstraete2004peps}.
%Much like the 1D case, these more complicated tensor networks also have cyclic group symmetries that reflect conservation laws in the operators.
%In both 1D and 2D contexts, effectively leveraging quantum symmetry reduces cost by a quadratic factor in the number of symmetry sectors, resulting in more than of order of magnitude affect on performance~\cite{}.
%In Section~\ref{sec:ex_tn}, we consider the most costly contractions arising in DMRG of a 1D tensor network, and the contraction of a PEPS (usually the main bottleneck in PEPS-based methods).
Tensor network (TN) methods represent a quantum state, and the associated operators  acting on it, as a contraction of tensors on the sites
of a lattice. %(\emph{sites}),
The contraction of the site tensors yields a full state or operator tensor with a number of modes
equal to the size of the lattice. % (i.e. an exponentially large number of entries in the size of the lattice).
%% Each site tensor is much smaller than the tensors directly describing the full state and operators, and the contraction of tensors
%%  formally encodes a
The simplest such tensor network is the
\emph{matrix product state (MPS)}~\cite{white1992density,fannes1992finitely} (also referred to as a \emph{tensor train}~\cite{oseledets2011tensor}), which is a 1D tensor network. It is widely used as part of the \emph{density matrix renormalization group (DMRG)}
method~\cite{white1992density,white1993density}.
DMRG uses an alternating optimization along the 1D tensor network to arrive at representations of ground or excited eigenstates of a Hamiltonian,
which is often itself represented as a tensor train (\emph{matrix product operator (MPO)}~\cite{verstraete2004matrix,crosswhite2008applying,chan2016matrix}).

Some common cyclic group symmetries in this context, known as Abelian quantum numbers, are those associated with
the magnetic spin quantum number and particle number symmetries (both $U(1)$ symmetries) as well as
fermionic supersymmetry ($Z_2$).
%% Physical Hamiltonians satisfy conservation laws, which result in cyclic group symmetries within the MPS and MPO.
%% Specifically, \emph{quantum number symmetries} may be used to represent conservation of ... ~\cite{}.
Tensor networks that go beyond a 1D contraction structure have substantially more expressive power~\cite{verstraete2004peps,vidal2008class,ye2018tensor}.
%One class defined in 2D and 3D (and which reduces to the MPS in 1D) is the \emph{projected entangled pair states (PEPS)} and associated operators (PEPOs), which provide a compact representation of the Hamiltonian eigenstates of physical interest in 2D and 3D~\cite{verstraete2004peps}.
%Tensor networks that go beyond a 1D contraction structure have substantially more expressive power~\cite{}.
The \emph{projected entangled pair states (PEPS)} are one such class defined in arbitrary dimensions (reducing to MPS in 1D)
and are believed to provide a compact representation of the Hamiltonian eigenstates of physical interest in higher dimensions~\cite{verstraete2004peps}.
These more complicated tensor networks exhibit the same cyclic group symmetries as found in matrix product states.
Because the symmetry groups arising in tensor network simulations can be arbitrary large (e.g. $U(1)$)
their efficient use can lead to orders of magnitude improvement in memory footprint and time to solution~\cite{white1993density,chan2002highly,mcculloch2002non,schmoll2020benchmarking}. Similarly to the situation in quantum chemistry, tensor contraction libraries
have been developed to handle these symmetries where the most common strategy is to track 
and loop over block-sparse representations~\cite{schmoll2020benchmarking,kao2015uni10,itensor,olivares2015ab}.
%% In both 1D and 2D contexts, effectively leveraging quantum symmetry reduces cost by a quadratic factor in the number of symmetry sectors, resulting in more than of order of magnitude affect on performance~\cite{}.
These contractions and block-sparse representations
can similarly be replaced by the cyclic group tensor representation
and irrep alignment algorithms of this work. In Section~\ref{sec:ex_tn}, we study two representative contractions: one arising in an MPS simulation using the DMRG algorithm, and one in
the contraction of a PEPS network.

